Visualizing Progress in Broadening Participation in Computing: The Value of Context

Concerns about representation in computing within the U.S. have driven numerous activities to broaden participation. Assessment of the impact of these efforts and, indeed, a clear assessment of the actual "problem" being addressed are limited by the nature of the most common data analysis which looks at the representation of each population as a percentage of the number of students graduating with a degree in computing. This use of a single metric cannot adequately assess the impact of broadening participation efforts. First, this approach fails to account for changing demographics of the undergraduate population in terms of overall numbers and relative proportion of the Federally designated gender, race, and ethnicity groupings. A second issue is that the majority of literature on broadening participation in computing (BPC) reports data on gender or on race/ethnicity, omitting data on students' intersectional identities. This leads to an incorrect understanding of both the data and the challenges we face as a field. In this paper we present several different approaches to tracking the impact of BPC efforts. We make three recommendations: 1) cohort-based analysis should be used to accurately show student engagement in computing; 2) the field as a whole needs to adopt the norm of always reporting intersectional data; 3) university demographic context matters when looking at how well a CS department is doing to broaden participation in computing, including longitudinal analysis of university demographic shifts that impact the local demographics of computing.

==> 00README.tex <==
nohypertex

